Evidence for a volcanic atmosphere on the sub-Earth L98-59b

Assessing the prevalence of atmospheres on rocky planets around M-dwarf stars is a top priority of exoplanet science. High-energy activity from M-dwarfs can destroy the atmospheres of these planets, which could explain the lack of atmosphere detections to date. Volcanic outgassing has been proposed as a mechanism to replenish the atmospheres of tidally-heated rocky planets. L 98-59 b, a sub-Earth transiting a nearby M dwarf, was recently identified as the most promising exoplanet to detect a volcanic atmosphere. We present the transmission spectrum of L 98-59 b from four transits observed with JWST NIRSpec G395H. Although the airless model provides an adequate fit to the data based on its $\chi^2$, an SO$_2$ atmosphere is preferred by 3.6$\sigma$ over a flat line in terms of the Bayesian evidence. Such an atmosphere would likely be in a steady state where volcanism balances escape. If so, L 98-59 b must experience at least eight times as much volcanism and tidal heating per unit mass as Io. If volcanism is driven by runaway melting of the mantle, we predict the existence of a subsurface magma ocean in L 98-59 b extending up to $R_p\sim 60-90\%$. An SO$_2$-rich volcanic atmosphere on L 98-59 b would be indicative of an oxidized mantle with an oxygen fugacity of $f\rm{O}_2>IW+2.7$, and it would imply that L 98-59 b must have retained some of its volatile endowment despite its proximity to its star. Our findings suggest that volcanism may revive secondary atmospheres on tidally heated rocky planets around M-dwarfs.

==> referee_report.tex <==
We thank the referee for a thoughtful and insightful report, which has helped improve the quality of this work. Below, we answer each of the referee's comments. Our changes to the manuscript are shown in bold. We also note that we have identified the issue regarding the extreme red noise originally present in the FIREFLy reduction of visit 2 NRS1: the spectroscopic fits (in which the non-linear polynomial coefficients are fixed to the white lightcurve values) were mistakenly pulling the 5th order white lightcurve coefficient instead of the 6th one. This issue is fixed in this new version of the paper.


1. Line 63: At what confidence has a circular orbit been ruled out? Is there any supporting new evidence that is stronger?
A: We have incorporated the most recent eccentricity measurement from the reanalysis performed by Rajpaul et al. (2024) of the 165 HARPS and 66 ESPRESSO spectra of L98-59. These data were originally published by Demangeon et al. (2021). The two measurements of the eccentricity are consistent with each other to 1 sigma. There are no additional radial velocity (RV) data listed on the ESO archive (as of January 2025). However, earlier papers also agree on a value of e~0.1 (Kostov et al. 2019), consistent with dynamical stability constraints (Cloutier et al. 2019). It is worth noting that even if the eccentricities were on the lower end of the quoted range, there would still be a large amount of tidal heating – several orders of magnitude per unit mass more than Io receives from Jupiter (Equation E1). While the tidal heating rate scales with eccentricity squared, due to the close proximity of the orbit (the heating rate scales as with period to the -5 power) if the eccentricity were orders of magnitude smaller there would still be more heating per unit mass than Io (assuming the same quality factor). 

2. Line 121: Very minor suggestion: technically there are more integrations in the observation if you count the target acquisition. Maybe just add "integrations per time-series observation" or "integrations per exposure"
A: We have changed "integrations per observation" to "integrations per time-series observation".

3. Line 82: Possibly consider citing the new paper by Dyrek+ on TRAPPIST-1 b
A: We are not aware of any paper by Dyrek et al. on TRAPPIST-1 b, but we have added a citation to Ducrot et al. 2024.

4. Line 156: Please clarify how this profile was constructed a little more. Would the 10-sigma temporal axis clipping remove any points in transit? Is the smoothing filter in the spatial or spectral axis?
A: We have clarified that the 10-sigma clipping is done to reject pixels that deviate by more than 10 sigma with respect to the median profile during optimal extraction. It should therefore not remove in-transit points, unless they are true outliers. The smoothing filter is performed along the spectral direction; we have added this information to the second paragraph of subsection 2.1. 

5. Line 166: Please clarify if long-frequency undulations have been seen in prior NIRSpec time series. It is more common in JWST lightcurves in the near-infrared to have a down-ramp.
A: We believe these undulations are due to the low number of groups per integration. We have added citations to Alderson et al. (2024) and Wallack et al. (2024), who reported similar time-correlated noise in NIRSpec data, and Hu et al. (2024) in NIRCam data. The data in all these works were taken with a low number of groups per integrations. Also, we have changed "long-frequency" to "low-frequency".

6. Line 184: Did the authors check that freely-fitted limb darkening coefficients were consistent with the ExoTiC-LD model?
A: Following the referee's comment, we performed an additional Eureka! reduction. In this new calculation, we fit for the limb-darkening coefficients instead of fixing them to the values from ExoTiC-LD. The resulting q1 and q2 values are shown in Fig. A3, and they are in agreement with the ExoTiC-LD model. In Fig. A1, we show that the resulting transmission spectrum is consistent with the original one. We have updated the text in Section 2.1 accordingly.

7. Line 197: If the authors fixed the quadratic term, was it consistent with a result where this quadratic term freely fit?
A: In this new version of the manuscript, we have produced an entirely new Eureka! reduction in which the quadratic term is freely fit. The resulting transmission spectrum is consistent with the one presented in the original manuscript. We show this in Fig. A1.

8. Line 248: Why is there no wavelength dependence to the limb darkening? I suggest a plot with the limb darkening used in the other analysis.
A: We appreciate the reviewer's suggestion. We have added Fig. A3, which shows a comparison between (i) the FIREFLy values, (ii) the ExoTiC-LD values (used in the Eureka! reduction), and (iii) the values we derived after fitting the limb-darkening coefficients. The ExoTiC-LD values are quite constant in this region (~0.1), and the value of q1=0.1 used by FIREFLy is consistent with the values derived from the fit. Meanwhile, the q2 values from ExoTiC-LD show no wavelength dependence, and the data places no constraints on q2 as evidenced by the flat posteriors. We have added this information to Section 2.2 and the Appendix.

9. Line 250: "we do not have to worry" sounds more like an opinion piece than a scientific paper. I suggest you show evidence or cite literature rather than this kind of language.
A: We have replaced that sentence by a reference to Fig. A3.

10. Line 266: A 6th order polynomial + x and y shifting is very high order and can lead to over-fitting transits. Have the authors considered using a Gaussian Process instead?
A: We thank the reviewer for pointing this out, and we agree that high-order polynomials can often result in over-fitting. In this case, the high-order polynomial is meant to capture changes at the beginning and end of the transit. The Eureka! reduction handled this by trimming some of the initial integrations, and the transmission spectra still agree, which points to the validity of both methods. Since we have approximately 2800 data points per lightcurve, we argue that a 6th order polynomial is still appropriate. While Gaussian processes can offer multiple advantages, they can affect the size of the uncertainties in the transmission spectrum (see Allen et al. 2024) and can also absorb the transit itself if strict priors are not used. Since we find that our 6th order polynomials fit the data well, we prefer to avoid the use of GPs in this case. 

11. Line 274: Linearity is not known to be time-dependent (to me). Do authors have a citation or evidence? Perhaps it could be stellar noise or electronic noise?
A: "Linearity" may be the wrong word to use here - we have replaced it with "precision". While we cannot rule out stellar or electronic noise, there seems to be a correlation between the amount of time-correlated noise in NIR JWST lightcurves and how few groups/integration there are. We have added this information to the text and included citations to relevant papers. 

12. Line 297: Does binning actually lead to more constraining models? Please justify this statement.
A: After looking into this, we found that in e.g. Moran et al. (2023), there are no significant differences in forward model constraints between reductions that bin according to equal wavelength vs. equal counts. We have removed this statement from the manuscript.

13. Line 342: Please list the number of degrees of freedom. I guess that it's 216, but if I'm not right, other readers will be wrong too.
A: That is correct: 216 degrees of freedom. We have added that number to the text.

14. Line 362: Please list the degrees of freedom for this chi-squared. Please also double check that the Bayesian evidence can be larger for the EPACRIS model (Chi-squared=198.7) than the airless model (197.84).
A: In the revised version of the manuscript, we decided to also include an inter-detector offset in both the volcanic atmospheres and the EPACRIS models (it was not included in earlier versions of either) to allow for a more fair comparison against the flat-line model. In this new version, the EPACRIS model has a lower chi2 (188.9). We have updated the chi2 values accordingly, and we now list the number of degrees of freedom in Section 3. 

15. Page 6: Figure 2. Put the bare-rock model here because this is referenced in many places.
A: We have added the bare-rock model to the plot.

16. Page 6: Figure 3. I suggest you over-plot abundances from the Seligman et al. 2024 paper or Aurora free retrievals.
A: We appreciate the reviewer's suggestion, but we do not think this is relevant to the main takeaway from Figure 3; in our self-consistent photochemical models the SO2 is assumed (rather than calculated). Moreover, the additional molecules listed that are produced by photochemical models are neither included as part of the retrievals or in the Seligman et al. (2024) paper. Finally, and unlike the retrievals or the Seligman et al. (2024) work, our photochemical models do not include CO2. Instead, they assume an SO2 dominated atmosphere because it is the only species that confidently appears in all retrievals.

17. Line 433: Clarify here why here the manuscript says no scenarios have enough significance over the baseline scenario? Did HST+JWST make the significance less than JWST alone?
A: Indeed, the sentence highlighted by the referee can be misleading. We meant to say that no scenarios had >5 sigma significance. In this new version, we have replaced that sentence by describing the scenario with the highest significance and mentioning the corresponding significance. Regarding the second question, the best-fit model is essentially flat at the HST wavelengths, but adding the HST data to the retrieval penalizes the evidence of the model, as it requires an additional free parameter (an offset). Nevertheless, the JWST and HST+JWST scenarios in Table A3 have slightly different free parameters, so it is hard to make a one-to-one comparison between them. In this new version of the manuscript, we list the number of degrees of freedom associated with each scenario (Table A3).

18. Line 520: What is the p-value? I recommend it be put in the abstract and/or conclusions.
A: We have added the p-value of the flat line (p=0.81) and all other models to this section. We also added the p-value of the flat line to the conclusions.

19. Line 569: Please repeat the number of degrees of freedom.
A: We have added the number of degrees of freedom (216) to the sentence.

20. Line 700: State explicitly what was done with aerosols. Were they excluded?
A: Our POSEIDON retrievals include a surface pressure free parameter. This parameter is designed to mirror the physical effect of an opaque cloud deck. The retrieval indicates that a wide range of surface pressures are possible ($P_surf>1E-5$ bar to 2 sigma), and therefore no high-altitude cloud is detected. We have added this information to the POSEIDON section.

21. Line 770: Please cite a reference for why these sulfur hazes don't form?
A: Sulfur hazes are self-consistently included in the photochemical model. These sulfur hazes do not form because the saturation vapor pressure increases quickly with temperature. We have added this explanation to Section 5.1.
 
22. Line 762: I am not sure this is the most likely explanation because the bare rock may be the simplest and still consistent scenario.
A: Indeed, the flat line is a simple model that provides an adequate fit to the data, and we cannot formally reject it. We have made a concerted effort to emphasize the fact that we do not reject the bare-rock model throughout the manuscript, including all subsections in Section 4 and the conclusions. The statement that the referee alludes to is based on the Bayesian evidence. Despite penalizing for the complexity of the atmosphere model, the Bayesian evidence still favors the SO2-rich atmosphere model over the flat line. The predictions from Seligman et al. (2024) provide supporting evidence. 

23. Line 765: I would suggest qualifying here that the discussion proceeds under the assumption that the SO2-rich scenario is correct.
A: We have included the following statement in the first paragraph of the discussion: "In this Section, we proceed under the assumption that the SO2-dominated scenario is correct."

24. Line 839: Most models have found that the fractionation of molecules via loss of lighter elements than heavier molecules is pretty weak (e.g. Burn et al. 2024). Please suggest a scenario how these could be consistent. Would an atmosphere with 90\% and 10\% SO2 be consistent with the data?
A: Our atmospheric retrievals disfavor CO2-rich atmospheres (CO2<84\% to 2 sigma, see POSEIDON section). However, a CO2-dominated atmosphere with a minor SO2 component (model 1 in Section 3.2) provides an adequate fit to the data based on its chi2, and therefore cannot formally be ruled out. We have added Fig. A4 in the appendix to show the retrieved SO2/CO2 abundance ratios from the Aurora retrieval. We note that the fractionation of elements depends strongly on the escape rate, which in turn depends on the efficiency. 

25. Line 900: The number of transits needed for a 5-sigma detection should be discussed elsewhere.
A: We have moved that paragraph to the Discussion.

26. Page 15: Figure A1. The wavelength binning scheme should be the same between the two pipelines (especially at overlapping wavelengths) for better inter-comparison.
A: We have updated FIREFLy's binning scheme in Fig. A1 to be equivalent to that of Eureka. 

27. Line 954: Could the offsets be due to stellar heterogeneities?
A: Stellar heterogeneities can certainly contribute to transit-to-transit variations in Rp/Rs. However, the fitted Rp/Rs values also vary significantly by reduction, pointing to correlated noise as the driver of these discrepancies. We have added this explanation to Section 2.2. 

28. Table A3. Please included the chi-squared per degree of freedom. As the text states, there can be some scenarios where the Bayesian evidence can be misleading so another metric will be helpful.
A: We have added the chi-squared, number of degrees of freedom, and reduced chi-squared values to all scenarios in Table A3.

29. Page 16: Figure A2. Please include ppm levels for the Allan deviation plots. Perhaps on the right Y axis?
A: We have changed the y axis to "RMS (ppm)" instead of "normalized RMS" for the white lightcurves the Allan deviation plots in Figure A2. We kept the "normalized RMS" y-axis in the case of the spectroscopic lightcurves. This choice was in order avoid the presence of Allan deviation lines with different vertical offsets. This would make the plots difficult to read and interpret because each of the Allan deviation lines have significantly different RMS values.

30. Page 16: Table A1. The difference between transit depths between pipelines is pretty significant for Transit 4 NRS2. Could it be the 6th order polynomial used?
A: Yes, this difference is almost certainly due to FIREFLY's choice of using a complex systematics model, which can obfuscate the true transit depth. We have emphasized this in Section 2.2.

